Analyzing Data-Centric Properties for Graph Contrastive Learning

Recent analyses of self-supervised learning (SSL) find the following data-centric properties to be critical for learning good representations: invariance to task-irrelevant semantics, separability of classes in some latent space, and recoverability of labels from augmented samples. However, given their discrete, non-Euclidean nature, graph datasets and graph SSL methods are unlikely to satisfy these properties. This raises the question: how do graph SSL methods, such as contrastive learning (CL), work well? To systematically probe this question, we perform a generalization analysis for CL when using generic graph augmentations (GGAs), with a focus on data-centric properties. Our analysis yields formal insights into the limitations of GGAs and the necessity of task-relevant augmentations. As we empirically show, GGAs do not induce task-relevant invariances on common benchmark datasets, leading to only marginal gains over naive, untrained baselines. Our theory motivates a synthetic data generation process that enables control over task-relevant information and boasts pre-defined optimal augmentations. This flexible benchmark helps us identify yet unrecognized limitations in advanced augmentation techniques (e.g., automated methods). Overall, our work rigorously contextualizes, both empirically and theoretically, the effects of data-centric properties on augmentation strategies and learning paradigms for graph SSL.

==> PAGES/inductive_bias_table.tex <==
\begin{table*}[ht]
 \centering
 \caption{\textbf{Benchmarking Graph URL Inductive Bias on Benchmark Datasets.} We report the performance of  \citep{You20_GraphContrastiveLearning}, GAE \citep{Kipf_VGAE}, AAGAE and SpecLoss against \textit{un}trained N-layer GIN encoders. Results for GraphCL are taken from the paper, while untrained model results are from \cite{Trivedi21_AugCL}. We use the same evaluation protocol and encoder architecture as \cite{You20_GraphContrastiveLearning} for trained models. Best results are indicated in bold; results within standard deviation are underlined.}
 \vspace{-0.3cm}
 \begin{adjustbox}{max width=\textwidth}
 \begin{tabular}{c c c  c c  c c c} 
\toprule
    \cmidrule(r){1-7}
  \textbf{Dataset}  & \textbf{Untrained (3)} & \textbf{Untrained(4) } & \textbf{Untrained (5)}  & \textbf{GraphCL}  & \textbf{GAE} & \textbf{AAGAE} & \textbf{SpecCL} \\
  \midrule
  MUTAG (188) & $\underline{85.76 \pm 7.38}$ & $\underline{86.36 \pm 6.51}$& $\underline{86.73 \pm 10.33}$  &  $\underline{86.80 \pm 1.34}$  & $\underline{87.76 \pm 3.00}$ & $\bm{88.23 \pm 0.98}$ & $\underline{86.17 \pm 4.11}$ \\
  PROTEINS (1113) & $\underline{73.64 \pm 5.464}$ & $\underline{74.46 \pm 4.09}$  & $\underline{74.22 \pm 2.85}$ & $\underline{74.39 \pm 0.45}$ & $\bm{75.36 \pm 0.4}$ & $\underline{74.77 \pm 0.43}$ & $\underline{74.00 \pm 1.58}$ \\
  NCI1 (4110) & $70.65 \pm 1.99$ & $70.36 \pm 3.11 $&  $70.49 \pm 2.42$ &  $77.81 \pm 0.41$ & $\underline{79.48 \pm 0.44}$ & $ \bm{79.75 \pm 1.25}$ & $76.66 \pm 0.029$  \\
  DD (1187) & $73.23 \pm 8.25$ & $ 72.15 \pm 7.25 $&  $\underline{77.08 \pm 4.18}$ & $\bm{78.62 \pm 0.40}$ & $\underline{78.24 \pm 0.67}$ & $\underline{77.59 \pm 0.64}$ & $\underline{78.43 \pm 1.18}$ \\
  RDT-B (2000) & $72.34 \pm 6.64$ & $64.57 \pm 8.03$ &  $67.32 \pm  7.41$ & $\bm{89.53 \pm 0.84}$ & $79.75 \pm1.25$ & $79.95 \pm 4.39$ & $79.28 \pm 1.049$ \\
  IMDB-B (1000) & $67.22 \pm 7.77$ & $61.26 \pm 7.01$ & $ 60.43 \pm 5.92$  & $\underline{71.14 \pm 0.44}$ & $\bm{71.70 \pm 0.36}$ & $\underline{71.26 \pm 0.305}$ & $\underline{71.4 \pm 2.19} $\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:statistics}
\end{table*}
